SneakyPrompt: Jailbreaking Text-to-image Generative Models

Text-to-image generative models such as Stable Diffusion and DALL$\cdot$E raise many ethical concerns due to the generation of harmful images such as Not-Safe-for-Work (NSFW) ones. To address these ethical concerns, safety filters are often adopted to prevent the generation of NSFW images. In this work, we propose SneakyPrompt, the first automated attack framework, to jailbreak text-to-image generative models such that they generate NSFW images even if safety filters are adopted. Given a prompt that is blocked by a safety filter, SneakyPrompt repeatedly queries the text-to-image generative model and strategically perturbs tokens in the prompt based on the query results to bypass the safety filter. Specifically, SneakyPrompt utilizes reinforcement learning to guide the perturbation of tokens. Our evaluation shows that SneakyPrompt successfully jailbreaks DALL$\cdot$E 2 with closed-box safety filters to generate NSFW images. Moreover, we also deploy several state-of-the-art, open-source safety filters on a Stable Diffusion model. Our evaluation shows that SneakyPrompt not only successfully generates NSFW images, but also outperforms existing text adversarial attacks when extended to jailbreak text-to-image generative models, in terms of both the number of queries and qualities of the generated NSFW images. SneakyPrompt is open-source and available at this repository: \url{https://github.com/Yuchen413/text2image_safety}.

==> Discussion.tex <==
\section{Possible defenses}


In this section, we describe several possible defenses that may be deployed by existing text-to-image models against the proposed \sys.  In general, we think the defenses can be divided into two major categories: (i) input filtering and (ii) training improvement. 

\subsection{Defense Type I: Input Filtering}

A common type of defense, which is deployed by existing text-to-image models like Stable Diffusion, is to filter input text prompts.  We describe two possible improvements on input filtering to defend against \sys below. 

\vspace{0.05in}
\para{Defense I-a: Token-level input filtering.} One possible defense is to enforce token-level input filtering instead of the sentence-level ones adopted by existing text-to-image models. Specifically, a defense could add a token-by-token embedding threshold, which will essentially block \sys because it can detect the sensitivity of the modified word instead of the whole sentence.  Therefore, the defense will better identify any possible word change that contributes to the generation of the final sensitive image.


\vspace{0.05in}
\para{Defense I-b: Meaningless word filtering.} Another simple, yet naive defense will be to enforce a word-level filter on meaningless words that are not found in any dictionaries, such as ``grponypui'' generated by \sys.  While this is very simple and effective in defending against some existing text-based adversarial examples (like ``n1ce''), no existing filters adopt such an approach. We would also like to note that advanced bypasses may still be possible if future researches enforce the word meaning as one of the constraints during search. 




\subsection{Defense Type II: Training Improvement}


Another type of defense is to improve existing text-to-image models during training.  This is generally harder than input filtering because it requires the heavy involvement of model owners to adopt such defenses. 

\vspace{0.05in}
\para{Defense II-a: Adversarial training.} 
 One possible defense, just like what people did for adversarial examples, is adversarial training, i.e., the inclusion of adversarial prompts in the training process of the safety filter (assuming it is learning-based) to harden the model's robustness.  Note that this is similar to the scenarios of existing adversarial examples, i.e., an adversary may still find new adversarial prompts, which bypass the safety filters while still preserving the semantics. 

 

\vspace{0.05in}
\para{Defense II-b: Sensitive concept removal. } Another possible defense is sensitive concept removal, e.g., via training data censorship.  That is, the trained learning model does not have any concepts related to sensitive content, and therefore it will not generate such images even given the target prompts.  This is also a challenging solution to adopt, because even if the model is unaware of the sensitive concept, a human being may describe the sensitive concept using other languages (e.g., red liquid vs. blood).  We believe that this will become important future works for researchers to tackle. 










